Bi-Directional Multi-Scale Graph Dataset Condensation via Information Bottleneck

Dataset condensation has significantly improved model training efficiency, but its application on devices with different computing power brings new requirements for different data sizes. Thus, condensing multiple scale graphs simultaneously is the core of achieving efficient training in different on-device scenarios. Existing efficient works for multi-scale graph dataset condensation mainly perform efficient approximate computation in scale order (large-to-small or small-to-large scales). However, for non-Euclidean structures of sparse graph data, these two commonly used paradigms for multi-scale graph dataset condensation have serious scaling down degradation and scaling up collapse problems of a graph. The main bottleneck of the above paradigms is whether the effective information of the original graph is fully preserved when consenting to the primary sub-scale (the first of multiple scales), which determines the condensation effect and consistency of all scales. In this paper, we proposed a novel GNN-centric Bi-directional Multi-Scale Graph Dataset Condensation (BiMSGC) framework, to explore unifying paradigms by operating on both large-to-small and small-to-large for multi-scale graph condensation. Based on the mutual information theory, we estimate an optimal ``meso-scale'' to obtain the minimum necessary dense graph preserving the maximum utility information of the original graph, and then we achieve stable and consistent ``bi-directional'' condensation learning by optimizing graph eigenbasis matching with information bottleneck on other scales. Encouraging empirical results on several datasets demonstrates the significant superiority of the proposed framework in graph condensation at different scales.

==> 4_problem.tex <==
% \section{Problem Analysis}
\section{Methodology}
% In this section, we theoretically analyze the main issues of the two multi-scale compression paradigms.

% Starting from the perspective of the gradient, there is an upper bound on its error:

% \begin{equation}
% \begin{aligned}
% \mathcal{L}_{GM}\leq&\|\mathbf{W}\|_{F}^{2}\|\mathbf{X}^{\top}\mathbf{A}^{2}\mathbf{X}-\mathbf{X}^{\prime}{}^{\top}\mathbf{A}^{\prime}{}^{2}\mathbf{X}^{\prime}\|_{F}^{2}\\&+\|\mathbf{X}^{\top}\mathbf{A}\mathbf{Y}-\mathbf{X}^{\prime}{}^{\top}\mathbf{A}^{\prime}\mathbf{Y}^{\prime}\|_{F}^{2},
% \end{aligned}
% \end{equation}

% where $\mathbf{X}^{\top}\mathbf{A}^{2}\mathbf{X}$ and $\mathbf{X}^{\top}\mathbf{A}\mathbf{Y}$ are two key distributions affecting the real map data. They play a crucial supervisory role in updating the synthetic map.

% $\mathbf{X}^\top\mathbf{u}_i\mathbf{u}_i^\top\mathbf{X}$

% Thereom 1: subset degredation problem:

% Thereom 2: growth boundary:

Initially, we present a theoretically integrated framework for multi-scale graph dataset condensation based on mutual information theory. Furthermore, we analyze the causes of multi-scale variation issues, including scaling down degradation and scaling up collapse, through the views of mutual information.

% \subsection{Graph Dataset Condensation in the Perspective of Mutual Information}
\subsection{Theoretical Understanding of MSGC}
According to the view of mutual information, the goal of the graph dataset condensation can be understood as :

\begin{equation}\max I\left(S_{sub};\nabla_{\theta}^{\prime}\right),\end{equation}

where $\nabla_{\theta}^{\prime}$ represents the valid information related to the original graph during model training. Specifically, in the gradient matching method, it refers to the gradient or the trajectory of the GNN training process. In the distribution matching method, it corresponds to the feature distribution.

For multi-scale graph dataset condensation, our goal is to ensure that each subset $S_{sub}$ of the maximum condensation scale graph $S$ retains the valid information required for model training. This can be represented as:

\begin{equation}\max I(S_{sub};\nabla_{\theta}^{\prime});\forall S_{sub}\in G_{sub}(S).\end{equation}

% That is, we want each subset to retain as much valid gradient information as possible. This process can be naturally translated into an information bottleneck objective. Specifically, the gradient information bottleneck is represented as:
% \begin{equation}\arg\max_{G_{sub}^S}I\left(S_{sub};\nabla_{\theta}^{\prime}\right)-\beta I\left(S_{sub};S\right),\mathrm{s.t.}S_{sub}\in\mathbb{G}_{sub}(S),\end{equation}
% \subsection{The reason for degeneracy and collapse problem }
\textbf{Understanding degeneracy and collapse problem.}
% The biggest challenge, however, is that we want good information retention at every scale possible. This provides a possible explanation for the potential problems with the two multi-scale distillation methods:
Based on experimental observations, we identify two key issues in multi-scale graph dataset condensation: scaling down degradation and scaling up collapse. We further analyze the dominating factors contributing to these problems using mutual information theory. For multi-scale graph dataset condensation $G_{sub}(S)=\{S_{1}, S_{2}, \cdots, S_{s}, \cdots, S_{m}, \cdots, S_{l}, \cdots, S_{max}\}$, where $S_i$ denotes the synthetic graph with a specific number of \textbf{N}odes \textbf{P}er \textbf{C}lass (NPC), $s$, $m$, and $l$ represent a small, medium, and large scale respectively. 

\textbf{Large to Small}: This method is designed to preserve the mutual information between the large-scale subset $S_l$ and the optimization objective, while progressively enhancing the mutual information for the small-scale subset $S_s$. However, when there is a significant difference in scale, the reduction in size leads to the loss of a substantial amount of node feature information. As the scale decreases, the model struggles to retain all the relevant data, inevitably resulting in the loss of some valuable compression information. This challenge highlights the difficulty of balancing information retention across varying scales, particularly when the disparity between large and small scales is pronounced.

\textbf{Small to Large}: This approach begins by preserving mutual information within small-scale graphs $S_s$, gradually introducing new training nodes to expand the scale and incorporate effective mutual information into the larger graph $S_l$. While this method effectively maintains a lower bound of mutual information retention at the smallest scale, it does not fully address the issue of scale discrepancy. As training progresses, the influence of the small-scale graph diminishes, and the optimization of the large-scale graph increasingly relies on the newly added nodes. This shift makes it challenging to retain effective information within the small-scale graph during the later stages of training. Furthermore, we observe that this approach can partially constrain the expressive power of the large-scale graph. This limitation may stem from the introduction of redundant information with the new nodes, which can dilute the overall effect and hinder the model's ability to fully leverage the potential of the larger graph.

Fortunately, we have identified an intermediate-scale condensation graph $S_m$ that effectively mitigates the loss of mutual information caused by scale differences. In addressing the scaling down degradation problem, this approach retains as much mutual information as possible while minimizing scale reduction. Conversely, in the case of scaling up collapse, it reduces the redundancy of extra information that often accompanies scale increases, thereby maintaining a more balanced and efficient compression process.


==> 9_checklist.tex <==
\section*{Reproducibility Checklist}
\begin{enumerate}
    \item This paper:
    \begin{itemize}
        \item Includes a conceptual outline and/or pseudocode description of AI methods introduced. {\color{blue}[YES]}  See Algorithm 1.
        \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. {\color{blue}[YES]}
        \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper. {\color{blue}[YES]}
    \end{itemize}

    \item Does this paper make theoretical contributions? {\color{blue}[Yes]}
    If yes, please complete the list below.
    \begin{itemize}
        \item All assumptions and restrictions are stated clearly and formally. {\color{blue}[YES]}
        \item All novel claims are stated formally (e.g., in theorem statements). {\color{blue}[YES]}
        \item Proofs of all novel claims are included. {\color{blue}[YES]}
        \item Proof sketches or intuitions are given for complex and/or novel results. {\color{blue}[YES]}
        \item Appropriate citations to theoretical tools used are given. {\color{blue}[YES]}
        \item All theoretical claims are demonstrated empirically to hold. {\color{blue}[YES]}
        \item All experimental code used to eliminate or disprove claims is included. {\color{blue}[YES]}
    \end{itemize}

    \item Does this paper rely on one or more datasets? {\color{blue}[YES]}
    If yes, please complete the list below.
    \begin{itemize}
        \item A motivation is given for why the experiments are conducted on the selected datasets. {\color{blue}[YES]}
        \item All novel datasets introduced in this paper are included in a data appendix. {\color{gray}[NA]}
        \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. {\color{gray}[NA]}
        \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. {\color{blue}[YES]}
        \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. {\color{blue}[YES]}
        \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. {\color{gray}[NA]}
    \end{itemize}

    \item Does this paper include computational experiments? {\color{blue}[YES]}
    If yes, please complete the list below.
    \begin{itemize}
        \item Any code required for pre-processing data is included in the appendix. {\color{blue}[YES]}
        \item All source code required for conducting and analyzing the experiments is included in a code appendix. {\color{blue}[YES]}
        \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. {\color{blue}[YES]}
        \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. {\color{blue}[YES]}
        \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. {\color{blue}[YES]}
        \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. {\color{blue}[YES]}
        \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. {\color{blue}[YES]}
        \item This paper states the number of algorithm runs used to compute each reported result. {\color{blue}[YES]}
        \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. {\color{blue}[YES]}
        \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). {\color{blue}[YES]}
        \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. {\color{blue}[YES]}
        \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. {\color{blue}[YES]}
    \end{itemize}
\end{enumerate}
